Sovereign Large Language Models: Advantages, Strategy and Regulations

This report analyzes key trends, challenges, risks, and opportunities associated with the development of Large Language Models (LLMs) globally. It examines national experiences in developing LLMs and assesses the feasibility of investment in this sector. Additionally, the report explores strategies for implementing, regulating, and financing AI projects at the state level.

==> abstract.tex <==
\begin{abstract}
Your abstract.
\end{abstract}

